Decentralized gradient methods: does topology matter?

Consensus-based distributed optimization methods have recently been advocated as alternatives to parameter server and ring all-reduce paradigms for large scale training of machine learning models. In this case, each worker maintains a local estimate of the optimal parameter vector and iteratively updates it by averaging the estimates obtained from its neighbors, and applying a correction on the basis of its local dataset. While theoretical results suggest that worker communication topology should have strong impact on the number of epochs needed to converge, previous experiments have shown the opposite conclusion. This paper sheds lights on this apparent contradiction and show how sparse topologies can lead to faster convergence even in the absence of communication delays.

==> bounds_self_contained.tex <==
%!TEX root = icml.tex

\begin{proof}
We rely on \citep[Thms 3, 4]{zeng18}. The bounds in Prop.~\ref{p:bounds} follow almost immediately once we prove that both the minimum level of our FJQN/B and the deterministic cycle time equal one.
We refer the reader to~\cite{zeng18} for the formal definitions of these two quantities and related ones.

In order to compute the level, one needs to first consider the circuit-free variant of the FJQN/B~\citep[Sect.~3.1]{zeng18}. In our case, because the initial marking has one job at each edge and the size of the buffers is $D+1>1$, the circuit-free variant is a new FJQN/B with graph $(\V\cup \V', \Ed')$, where $\V'$ is a new set of $|\Ed|$ nodes, one for each edge in the original graph. We indicate the node in $\V'$ corresponding to edge $(i,j)\in \Ed$ as $u'(i,j)$. The set of edges $\Ed'$ is defined as follows: $\Ed' =\{(i,u'(i,j))\;\;  \forall (i,j) \in \Ed  \} \cup \{(j,u'(i,j))\;\;  \forall (i,j) \in \Ed  \}$. Buffer sizes are equal to $b^- = 1$ for the first set of edges and to $b^+ = D$ for the second group.
We observe that the graph $(\V\cup \V', \Ed')$ is bipartite, with links only from the original nodes in $\V$ to nodes in $\V'$. It follows that the function $l: \V \cup \V' \to \mathbb N$, such that $l(v)=1$ if $v\in \V$ and $l(v)=2$ if $v\in \V'$ is trivially the optimal topological labelling~\citep[Sect.~4.1]{zeng18} of the graph with maximum label gap over the edges equal to $1$. Then the minimum level associated to our FJQN/B is indeed $1$.

For the deterministic cycle time, we need to consider the deterministic non-blocking variant of our FJQN/B~\citep[Sect.~3.2]{zeng18}. The corresponding graph has the same set of nodes $\V$. The set of edges is increased by adding for each edge in $\Ed$ a reversed edge with initial marking equal to the number of holes in the original edge, and a self-loop edge for each node with initial marking equal to one job. Because in our case $\E{\tau}=1$, the deterministic cycle time can then be computed as 
$\max_{\xi \in \Xi}\frac{S(\xi)}{J(\xi)}$,
where $\Xi$ is the set of all the circuits\footnote{
A path is a sequence of directed contiguous edge, i.e., $(i_1,i_2)$, $(i_2, i_3)$, \dots $(i_{l},i_{l+1})$ with $(i_h,i_{h+1}) \in \Ed$ for each $h=1, 2, \dots l$. A circuit is a path with $i_{h+1}=i_1$.
} in the deterministic non-blocking  variant, $S(\xi)$ and $J(\xi)$ denote respectively the number of nodes and  the total number of jobs in the circuit $\xi$.
In our case every edge has at least one job, so that the cycle time is at most one, but this bound is achieved on any circuit made by the original edges. We conclude then that the deterministic cycle time for our FJQN/B is indeed $1$.



\end{proof}

==> rate_existence_self_contained.tex <==
%!TEX root = icml.tex

\begin{proof}
We start proving that the FJQN/B of our system is necessarily deadlock-free~\citep[Def. 4.2]{dallery94}, that means, roughly speaking, that it is not possible that all nodes are blocked or starved at a given time. 
%We need to introduce some terminology. 
%A path of length $l$ is a sequence of directed contiguous edge, i.e., $(i_1,i_2)$, $(i_2, i_3)$, \dots $(i_{l},i_{l+1})$ with $(i_h,i_{h+1}) \in E$ for each $h=1, 2, \dots l$. A circuit is a path with $i_{h+1}=i_1$.  Similarly 
We define a chain of length $l$ to be a sequence of undirected contiguous edges, i.e., $(i_1,i_2)$, $(i_2, i_3)$, \dots $(i_{l},i_{l+1})$ with $(i_h,i_{h+1}) \in E$ or $(i_{h+1}, i_h) \in E$ for each $h=1, 2, \dots l$. A cycle is a chain with $i_{h+1}=i_1$.
Consider the system at time $0$. Given a cycle
%\footnote{ Please refer to \cite{dallery94} for the definition of a cycle.}
 $\mathcal C$ of length $l$, define an arbitrary orientation of it. Let $I_+(\mathcal C)$ denote the total number of jobs in all the buffers on edges that are oriented according to the reference orientation plus the total number of holes (places available) in all the buffers on edges that are oriented according to the reverse direction. Given that the initial marking of our FJQN/B has a single job in any buffer, it follows
\[l \le I_+(\mathcal C) \le l (B-1), \]
where $B(=D+1)$ is the size of each buffer. The lower (resp. upper) bound corresponds to the case where all the edges in the cycle are oriented according to the reference (resp. reverse) direction. Being that $0< I_+(\mathcal C) < l B$ for each cycle, it follows from \citep[Theorem~4.1]{dallery94} that the FJQN/B is deadlock-free.


We now observe that 
\[ \lim_{t \to \infty} \frac{t}{\lfloor s_i(t)/2 \rfloor} = \lim _{t \to \infty} \frac{t}{\lfloor \min_i s_i(t)/2 \rfloor}, \]
if any of them exists.
Moreover, for any deadlock-free FJQN/B it can be checked that 
%\[\frac{T_i(k)}{k} \le \frac{t} {\lfloor s_i(t)/2 \rfloor} < \frac{n+1}{n} \frac{T_i(k+1)}{k+1},  \]
%and similarly
\[\frac{\max_i T_i(k)}{k} \le \frac{t} {\lfloor \min_i s_i(t)/2 \rfloor} < \frac{k+1}{k} \frac{\max_i T_i(k+1)}{k+1}.  \]
Then, if  $\lim_{k\to \infty} \frac{\max_i T_i(k)}{k}$ exists,   $\theta$ exists and is equal to such limit. The result then follows from~{\citep[Thm.~5.2]{dallery94}}.



\end{proof}

==> related.tex <==
%!TEX root = icml.tex
In the parameter server framework, workers can use stale versions of the model to compute ``delta'' updates of the parameters, that are then aggregated by the parameter server. % and combined with its current state.  
If model parameters can be arbitrarily old, the system works completely asynchronously, its throughput increases, but convergence to the correct minimizer is not guaranteed in general.  If  staleness is not tolerated, parameters are updated as in the clique topology considered in this paper.
%The most recent versions of parameter server architecture allow the programmer to specify a bound on the staleness of the parameters values used by the workers.
By imposing a bound on the staleness of the parameter values used by the workers, the programmer %most recent versions of parameter server architecture 
can trade solution quality off against convergence speed~\cite{ho13,li14nips}. 

Consensus-based optimization schemes also mitigate the effect of stragglers through a form of inconsistency: rather than a chronological one (workers use versions of the same parameter vector but with different ages),  it is a \emph{spatial} one (workers are allowed to maintain different parameter vectors). %, but work on the most recent version from their neighbours). 
It can be shown that the difference between current iteration numbers at two workers in DSM is bounded by the diameter of the graph. The diameter then plays the same role of the staleness threshold in the parameter server: %Similarly to what happens for the staleness threshold, 
the larger the diameter, the higher the throughput, but local parameter vectors can be farther from each other and from the minimizer. Our paper shows that the first effect overwhelms the second. The two straggler mitigation techniques (chronological and spatial) are orthogonal and can be  used jointly. %, a possibility that we plan to investigate in the feature.

Surprisingly, much of the existing literature on distributed optimization algorithms has ignored the effect of network connectivity on convergence speed, because it considered the underlying network topology to be imposed by specific communication constraints (e.g., sensors' limited transmission range). The few exceptions~\cite{nedic18,duchi12} suggest that the all-to-all communication pattern is preferable, unless it causes communication delays to increase~\cite{tsianos13}. 
Similary,~\cite{lian17nips,lian18icml} recently observed that if the parameter server becomes the communication bottleneck, then other communication patterns can be more advantageous.
 In this paper we show that a sparse topology may be preferable even when communication times are negligible. When not negligible, the improvement from sparse topologies is even larger.


ASAP~\cite{kadav16} is a distributed framework that proposes a form of fine-grained synchronization, which can support our consensus based gradient method. 
%The framework is developed in C\texttt{++} and provides Lua bindings to run existing Torch and RAPID deep learning networks.
Experimental results on an infiniBand implementation stack show that degree-3 expanders  can achieve up to 2-10X speedups to train SVM methods as well as  convolutional neural networks. Our theoretical results contribute to understanding the observations in~\cite{kadav16}, and their experiments further support that our conclusions also hold for non-convex optimization problems.

%We observe that another advantage ofThis all-to-all communication scheme does not reflect the fact that large statistical models are often composed of different submodels only loosely dependent on each other~\cite{low12}. Accounting for submodel dependencies to design  communication flows between the computing nodes can result in a significant decrease of network traffic. Moreover, specific communication patterns may be beneficial in heterogeneous clusters 
%or required by organisational constraints. % (e.g., when multiple learners do not want necessarily to share the datasets). 
%For these reasons, the new abstract paradigm CoCoA~\cite{smith18}, and the  full-fledged ML systems GraphLab~\cite{low12} and  TensorFlow~\cite{abadi16} advocate the need for more flexible communication patterns, e.g.,~using general dataflow graphs to represent computation. 
%
%In particular, in TensorFlow Graphs, nodes are computing units, which communicate through edges.  Each node receives $n$-dimensional arrays (tensors) as inputs through its incoming edges, processes them and produces new tensors that are transmitted on its outgoing edges. Each edge is associated with a queue that stores the tensors. Several queueing policies are implemented (FIFO, Random, Priority) to support advanced forms of coordination. 



==> speed.tex <==
%!TEX root = icml.tex
References~\cite{tsianos13,lian17nips,lian18icml} suggest that, when network delays are accounted for, topologies with small per node communication load (e.g.,~sparse permutation invariant graphs) can achieve smaller convergence times. In this section, we show that this is the case even when there is no communication delay, but there are stragglers, i.e.,~nodes exhibit variable computation times.

The convergence time of an iterative ML algorithm ($T_\epsilon$) depends both on the number of iterations ($K_\epsilon$) required to achieve a solution with precision~$\epsilon$ %of acceptable quality 
and on the average time required to carry out one iteration ($\theta$). As a first approximation, $T_\epsilon = K_\epsilon \times \theta$. This simple relation expresses an important quality vs quantity trade-off, because the connectivity of the dataflow graph has an opposite effect on each of the quantities $K_\epsilon$ and $\theta$. As we saw in the previous section, the less connected is the topology, the less informative is each iteration and the more iterations are required ($K_\epsilon$ increases). At the same time, each iteration is faster ($\theta$ decreases), because each node is less dependent on other nodes and spends less time waiting for inputs and more time computing. The topology of the dataflow graph then affects system  throughput, i.e.,~how many iterations per time unit the system is able to complete. Given a dataflow graph $\G$ and $\G'$ a subgraph of $\G$, we expect a higher throughput for the less connected $\G'$. If computation times are independent and identically distributed random variables, this relation can be formally established through a coupling argument. 

Under the same i.i.d.~assumption on the computation times, DSM operation can be described as a fork, join, queueing network with blocking (FJQN/B)~\cite{dallery94}. A  FJQN/B is a queueing network that can be represented by a directed graph where nodes are servers and buffers are associated with edges. In general, a server has multiple input buffers on the incoming edges and multiple outgoing edges. A server is allowed to start service whenever there is at least one job in each of its input buffers and space for at least one job in each of its output buffers. Upon completion of service at a node, one job is removed from each of its input buffers and one job is added to each of its outgoing buffers. 
%A complete description of a FJQN-B requires specifying, besides the buffer sizes and service time distributions, an initial ``marking,'' i.e.,~the number of jobs in each buffer at time~$t=0$.
%, as well as the initial ``timing'' condition, i.e.,~after how much time after $t=0$ each server can start its service.
The parallelism between the descriptions of TensorFlow Graphs and FJQN/B is evident.
It is easy to check that  our system can be represented as a FJQN/B where a job in the buffer at link $(i,j)$ maps to an estimate $\x_i$ computed by node $i$, but not processed yet by node $j$.
%, that has not still processed it. 
%In particular, the graph associated to the FJQN/B is $\mathcal G$ itself, the initial marking has one job at each buffer, 
%%all the timing values are zero (nodes can immediately start computing), 
%and buffer sizes can be set equal to $D+1$.\footnote{
%	This value guarantees that there is no buffer blocking in the system but only synchronization blocking.}
	
Relying on results on FJQNs and in particular on {\citep[Thms 3, 4]{zeng18}}, it is possible to establish that  the average iteration time $\theta$ 1) is well defined, and 2) satisfies the following bounds (see~\citeapp{a:throughput}):
%Recent papers on FJQN/B also allow us to derive bounds for $\theta$. The bounds in~[Theorems~3,~4]\cite{zeng18} depend on the ``minimum level'' and the ``deterministic cycle time'' (respectively $L^*$ and $c$ in \cite{zeng18}). We do not provide here their definitions, we just observe that both values depend in general on the graph $\G$ and on the initial marking. In our case they happen to be both equal to $1$. This observation and the buffer value established above lead to the following bounds, whose proof is in~\citeapp{a:iteration_time}
\begin{prop}
\label{p:bounds}
If computation times are bounded from above by $\tau_{\max}$, the following holds:
\begin{equation}
\label{e:bound_bounded}
1 \le \theta \le 4 \tau_{\max}.
\end{equation}
If they are unbounded but have finite moment generating function $M_{\tau}(t)$, the following holds:
\begin{equation}
\label{e:bound_unbounded}
\max\left(1,\frac{\E[\tau_{(d)}]}{D}\right)\le \theta \le \frac{\frac{2 \ln(4 d M_{\tau}(t))}{D}+\ln(M_\tau(t))+\ln 2}{t/2},
\end{equation}
for any $t>0$ such that $M_\tau(t)<\infty$.
\end{prop}
%\input{bounds_self_contained.tex}

%If computing times are exponentially distributed with expected value $1$, $M_{\tau}=1/(1-t)$.  
Here, $D$ is the diameter of the graph.
For a directed cycle with $M$ nodes and exponentially distributed computing times with rate $1$ ($d=1$, $D=M-1$, and $M_{\tau}(t)=1/(1-t)$), the bound (\ref{e:bound_unbounded}) %then predicts that
%we know that the iteration time is smaller  $\theta_{\textrm{cycle}}\le \theta_\textrm{clique}$, but   can be used to find a better upper bound. Observe that for a cycle 
%. Then, it holds:
%\[\theta_{\textrm{cycle}} \le \inf_{0 < t < 1}\frac{ \left(1+\frac{2}{M-1}\right) \ln \frac{1}{1-t}+ \left(1+\frac{4}{M-1}\right) \ln 2 }{t/2}. \]
predicts that $\theta_\textrm{cycle} \le 5.35$ for large $M$.
%For large $M$, this gives $\theta_\textrm{cycle} \le 5.35$. 
Instead, for a clique, every worker needs to wait for all the others and then it is  $\theta_\textrm{clique} = \max(\tau_1, \dots \tau_M)= \sum_{i=1}^M \frac{1}{i} \approx \ln M $. 
This result shows that the cycle is not only faster than the clique, but, asymptotically, arbitrarily faster. 

The results in this section and in the previous one suggest that sparser dataflow graphs may  lead to shorter ML training periods. The final balance between the two opposing effects of topology on iteration quality and iteration throughput depends on dataset characteristics and computing time distribution. In the next section we show that,  in realistic ML experiments, sparse topologies can indeed be preferable.




==> table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Data& Model& M& bsz& $\sqrt{\frac{E}{E_{sp}}}$& $\frac{\sqrt{E}}{H}$ & $\frac{1}{\alpha(1)}$ & $\gamma$ & $||\nabla F||^2$ & $||\sigma||^2$ \\
\hline 
\multirow{4}{*}{ \begin{tabular}{c}CT\\ (52000)\end{tabular}}& 
\multirow{4}{*}{ \begin{tabular}{c}Linear\\ n=384\end{tabular}}& 
\multirow{2}{*}{16}        &  &  & &  &  & & \\
            & &            &  &   &       &    &  &  &\\ 
&&\multirow{2}{*}{100}     &  &  & & & &  & \\
& &                        &  & & & & & & \\
\hline
\multirow{4}{*}{ \begin{tabular}{c}MNIST\\ (60000)\end{tabular}}& 
\multirow{4}{*}{ \begin{tabular}{c}2-conv Layers\\ n=476170\end{tabular}}& 
                 10*    &128 &1.01 & 1.00 &1.43 & 1.43&   &\\
  & &                 16      &128 & 3.52 &1.05 &1.49 & 5.51&   &\\
    & &                 16  &1000 & 3.52 &1.05 &1.49 & 5.51&   &\\
&&64    & 128  & & & & & & \\
\hline
\multirow{2}{*}{ \begin{tabular}{c}CIFAR10\\ (50000)\end{tabular}}& 
\multirow{2}{*}{ \begin{tabular}{c}ResNet18\\ n=11220132\end{tabular}}& 
\multirow{2}{*}{16}        &128  &1.10& & & 1.49 && \\
            & &          &   512  & & & & & &  \\ 
\hline

\end{tabular}

==> toy_example.tex <==

In this section we consider a toy example to illustrate the implications of the findings in the previous section. 
We want to solve the following problem:
\begin{align}
& \minim_w & & F(w)=\frac{1}{M}\sum_{l=1}^M 1 - y^{(l)}  x^{(l)} w \label{e:toy_problem}\\
& \textrm{subject to} & & w \in \sW\nonumber
\end{align}
%This function is often used for Support Vector Machine (SVM) classification 
where $x^{(l)}$ is a data feature and $y^{(l)} \in \{-1,1\}$ identifies the class label. Note that there is only one parameter $w \in \mathbb R$ ($n=1$) and, for the moment, the number of nodes equals the size of the dataset ($M=m$). 
%We compare these results with our theoretical findings in the previous sections. 
$\Delta \mG(k) = \mG(k) - \mG(k) \frac{\vone \vone^\intercal}{M}$ is in this case a constant row vector.
    

\begin{figure*}[h]
%\vspace{.3in}
        \centering
        \begin{subfigure}{0.3275\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test1_eigvecsvm_100n_err_vs_iter.png}
            \caption%
            {{\small Rings with aligned gradient}}    
            \label{f:rings}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.3275\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test2_eigvecsvm_100n_err_vs_iter.png}
            \caption%
            {{\small Expanders with aligned gradient}}    
            \label{f:expanders}
        \end{subfigure}
        %\vskip\baselineskip
        \hfill
        \begin{subfigure}{0.3275\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test3_eigvecsvm_100n_err_vs_iter.png}
            \caption%
            {{\small Expanders with generic gradient}}    
            \label{f:no_alignment}
        \end{subfigure}
%        \quad
%        \begin{subfigure}[b]{0.475\textwidth}   
%            \centering 
%            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test4_eigvecsvm_100n_err_vs_iter.png}
%            \caption[]%
%            {{\small Network 4}}    
%            \label{fig:mean and std of net44}
%        \end{subfigure}
	%\vspace{.3in}
        \caption[ ]
        {\small Objective function~(\ref{e:toy_problem}) evaluated for the worst model $\vw_j(k)$ versus number of iterations: effect of the topology and its relation with the gradients.} 
        \label{f:gradient_and_topology}
    \end{figure*}

    \begin{figure*}[h]
    	%\vspace{.3in}
        \centering
        \begin{subfigure}[b]{0.3275\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test4_multieigvecsvm_100n_2samples_err_vs_iter.png}
            \caption[]%
            {{\small 2X dataset}}    
            \label{f:similar_gradients2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3275\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test4_multieigvecsvm_100n_20samples_err_vs_iter.png}
            \caption[]%
            {{\small 20X dataset}}    
            \label{f:similar_gradients20}
        \end{subfigure}
        %\vskip\baselineskip
        \hfill
        \begin{subfigure}[b]{0.3275\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test4_multieigvecsvm_100n_100samples_err_vs_iter.png}
            \caption[]%
            {{\small 100X dataset}}    
            \label{f:similar_gradients100}
        \end{subfigure}
%        \quad
%        \begin{subfigure}[b]{0.475\textwidth}   
%            \centering 
%            \includegraphics[width=\textwidth]{figures/simulations_wide_layout/test4_eigvecsvm_100n_err_vs_iter.png}
%            \caption[]%
%            {{\small Network 4}}    
%            \label{fig:mean and std of net44}
%        \end{subfigure}
	%\vspace{.3in}
        \caption[]
        {\small Objective function~(\ref{e:toy_problem}) evaluated for the worst model $\vw_j(k)$ versus number of iterations: effect of dataset size. Expanders with generic gradient.} 
        \label{f:similar_gradients}
    \end{figure*}



%The datasets are generated as follows.
%We start from a vector $\vu$ of values in $[-1,1]$ which sum up to zero. % ($\vu^\intercal \vone=0$). 
%We describe later how the vector $\vu$ is selected in the different experiments. Features $x^{(l)}$ are defined as $x^{(l)} = |u_l+\zeta|$, where $\zeta$ is a small positive constant. The labels are defined as $y^{(l)}=-\sign(u_l+\zeta)$. We select $\sW=[-30,1]$. Observe that $F(w) = 1 - \sum_l y^{(l)} x^{(l)}/M = 1 + \zeta w$,
%%$F'(w)= -M^{-1} \sum_l y^{(l)} x^{(l)} =  \zeta+ M^{-1}\sum_l u_l  = \zeta>0$, 
%and consequently the minimizer of problem~(\ref{e:toy_problem}) is $w^*=-30$. We select $\zeta=1/10$, $\eta(k)= 1/10$ and all nodes start with the same initial estimate $w_i(0)=1$.


We consider an undirected $d$-regular graph with $M=100$ nodes and homogeneous  non-negative weights, i.e.,~$A_{i,j}=1/(d+1)$ for $(i,j) \in \Ed$ and $A_{i,j}=0$ otherwise. Matrix $\mA$ is then symmetric. 

%Our numerical results have been obtained through a discrete event simulator developed in Python. 




%Fig.~XXX~a) shows a  typical dataset used for the next experiment. 
%is positive if and only if positive labelled samples have a larger mean than negative labeled ones. In the datasets $x^*<0$, because $\sum_l$.
%Let $J^+$ (/$J^-$) be the samples belonging to class $+1$ (/$-1$). The two classes have the same number of elements. The minimizer $x^*$ of \eqref{e:simple_svm}  is positive if and only if positive labelled samples have a larger mean than $ \sum_{l\in J^+}  \vx^{(l)} >  \sum_{l\in J^-} \vx^{(l)}$. the average feature value for samples of nodes with a positive label have  of  simple case the optimal value $x^*$ will be positive 
%where $\chi$ is the feature value and $y$

%\paragraph{Bound XXX is tight.}
Figure~\ref{f:rings} presents results for undirected $d$-regular rings, where each node $i$ %$ \in \{0, \dots M-1\}$ 
is connected to nodes $i-1$ and $i+1$ (hence forming a cycle) as well as the $d-2$ closest nodes  on the cycle.
%: for $d$ even, to nodes  $\{i-d/2, i-d/2+1, \dots, i-2, i+2, \dots, i+d/2-1, i+d/2\}$, for $d=3$,  to $i+2$ or $i-2$.
%For $d$ even, $i$ is connected to nodes  $\{i-d/2, i-d/2+1, \dots, i-2, i+2, \dots, i+d/2-1, i+d/2\}$. For $d=3$, node $i$ is connected to $i+2$ or to $i-2$.
%i.e., in the set $\{i-d, i-d+1, \dots, i-2, i+2, \dots, i+d-1, i+d\}$ (sum and differences are module $M$).
Among graphs with degree~$d$, these rings are poorly connected, with a diameter that is order of $M/d$ and low spectral gap $1-|\lambda_2|$. 
The curves show the evolution of the objective function evaluated at the worst estimate, i.e.,~$\max_i F(\hat w_i(k))$ %, across different iterations 
for different values of the degree $d$.
For each degree, the dataset is chosen perturbing a left eigenvector ($\vu$) of $\mA$ relative to $\lambda_2$ by a small quantity $\zeta>0$ so that 1) local gradients are very different ($\Lsp \ge 1 = L$) and 2) $\Delta \mG(k) = \vu^\intercal$. When $\Delta \mG(k) = \vu^\intercal$ holds, we say that gradients are \emph{aligned with the topology}.\footnote{
	It corresponds to the slowest convergence scenario for distributed dual averaging, see~{\citep[Prop.~1]{duchi12}}.
} All the energy of $\Delta\mG(k)$ is in the subspace defined by $\mP_2$, then $\alpha(1)=\sqrt{e_2}=1$. Details about how the dataset is built are in \citeapp{a:toy_example},  together with calculations showing that  the value of the objective function~is 
\begin{align}
 \max_i & (F(\hat w_i(k-1)))  = \nonumber\\
	& = 1 +  \zeta + \frac{  \eta \zeta}{1-\lambda_2} \left( 1- \frac{1- \lambda_2^{k}}{k(1-\lambda_2)}\right) -  \eta  \zeta^2 \frac{k}{2}. 
\label{e:toy_worst}
\end{align}
Equation (\ref{e:toy_worst}) exactly matches the plots in Fig.~\ref{f:rings}. 
Comparing~(\ref{e:toy_worst}) with~(\ref{e:classic_bound}) and~(\ref{e:new_bound}), we recognize the same dependence on the second largest eigenvalue.\footnote{
	Equation~(\ref{e:toy_worst}) indicates a much faster convergence than those bounds, because, for simplicity, we considered a differentiable linear objective function~\eqref{e:toy_problem}.
} 
Because $\Lsp \ge L$ and $\alpha(1)=1$,  the two bounds~(\ref{e:classic_bound}) and (\ref{e:new_bound}) are almost equivalent, but for the fact that~(\ref{e:new_bound}) correctly takes into account that there is no dependence on the initial estimates ($\Rsp=0$). % because all the nodes start from the same local model $\Rsp$.

Figure~\ref{f:rings} shows clearly a high variability of the performance of the optimization algorithm across different topologies. The number of iterations required to achieve a given approximation of the optimum is orders of magnitude larger for the cycle ($d=2$) than for the clique ($d=99$).

In Fig.~\ref{f:expanders} the same experiments are executed on $d$-regular connected random graphs. These graphs are known to be Ramanujan graphs with high-probability, i.e.,~they have the % largest possible spectral gap  
smallest $|\lambda_2|$ among all graphs with the same degree~\cite{mckay81}. The curves still follow~(\ref{e:toy_worst}), but because $\lambda_2$ is  smaller, objective function $F(\cdot)$ takes on smaller values. Note that the curves for $d=2$ and $d=M-1$ are unchanged, because the corresponding graphs are always the same (the cycle and the clique, respectively). We also observe that the relative performance differences  for graphs with $d\ge 3$ are much smaller:  the marginal benefit to increase connectivity is much less for random graphs.



Until now, we have assumed  that row matrix $\Delta\mG$ is aligned with a left eigenvector of $\mA$, but there is no particular reason to think this should be the case. Figure~\ref{f:no_alignment} shows numerical results for the case when the same datasets as in Fig.~\ref{f:expanders} are used, but the graph is a new  independently generated $d$-regular random graph.\footnote{
	For the case $d=2$, the original dataset is randomly distributed across the nodes.
} %are generated, independently from those used to generate the datasets.
In the figure, we see that connectivity is even less important and that the curve for $d=2$ starts approaching the others. This experiment shows the effect of $\alpha(1)$. $\vu$ is the most difficult configuration to average for the consensus matrix $\mA$. Now vector $\Delta\mG$ and the vector $\vu$ %of $\mA$ %corresponding to $\lambda_2$ 
are arbitrarily oriented, so that on average only $(1/M)$th of the energy of $\Delta\mG$ falls in the direction of~$\vu$.

%Another way to quantify this effect is to look at the norm of the perturbation vector $ \vu^{\intercal} \frac{1- \lambda_2^k}{1-\lambda_2}$

%We look now at the effect of $\Lsp$. 
We now look at how gradient variability affects convergence.
%In the experiments  the local gradient  $\vg_i$ at node~$i$ is equal to $u_i+\zeta$, where $u_i \in [-1,1]$ so nodes have very different local gradients. 
%and the differences $\vg_i - \bar \vg$ are equal to $u_i$ so they are spread over $[-1,1]$. 
We increase the dataset size and have each node compute its local function on the basis of more data samples. The additional data is built as above from the second eigenvectors of new  independently generated $d$-regular random graphs. The new data have then the same statistical properties. Figure~\ref{f:similar_gradients} shows what happens %for dataset sizes 2, 20, and 100 times larger, and 
when each node stores respectively 2, 20, and 100 data points.  Because the local datasets become more and more similar as dataset size increases, $\Lsp$ reduces and the curves get closer and closer. For a $100$x dataset,  the convergence rate of a cycle ($d=2$) differs little from that of a fully connected graph.



%Finally, problem~(\ref{e:toy_problem}) is a linear one, where the gradient  always has the same module. In a realistic case, where DSM approaches a minimizer of the function $F$, we expect the module of the gradient to progressively decrease. In (\ref{e:new_bound}) this  corresponds to $L$ and $\Lsp$ becoming progressively smaller. As an example, consider the following modification of the objective function~(\ref{e:toy_problem}):
%\begin{equation}
%F(w)=\frac{1}{M}\sum_{l=1}^M \max(0, 1 - y^{(l)}  x^{(l)} w),
%\label{e:simple_svm}
%\end{equation}
%where we  recognize that the local functions are simple one-dimensional hinge loss functions.
%%The optimization starts from $w_i(0)=1$ for each $i$ and then the $\max$ operator has no effect at the first step. As $w_i(k)$  decreases, the local functions at nodes for which $-y^{(l)} x^{(l)}$ is negative will progressively become $0$ because of the $\max$, and finally their local subgradient will be null. 
%Figure~\ref{f:gradient_module} shows the objective function with the same dataset and configuration of Fig.~\ref{f:similar_gradients100}. After  $2000$ iterations, the effect of different topologies is negligible.
%
%
%\begin{figure}
%%\vspace{.3in}
%\centering
%\includegraphics[width=0.3275\textwidth]{figures/simulations_wide_layout/test5_multieigvecsvm_100n_100samples_err_vs_iter.png}
%%\vspace{.3in}
%\caption{Objective function~(\ref{e:simple_svm}) evaluated for the worst model.}
%\label{f:gradient_module}
%\end{figure}




%Pareto computation times with $\sigma= 2$ and $\beta=3$ and  expander topologies\footnote{
%	The topologies have been selected by generating a large number of regular connected random graphs with the same degree using the function ZZZ in network X and then selecting among them the one leading to the largest spectral gap.
%} with different degrees. In particular, Fig. YYY~a) shows the total number of iterations versus time. We see that, as expected, sparser networks lead to faster iterations and in particular our model XXX predicts quite well the effect of the different degrees as already observed in Sect.~XXX. The curves in Fig. YYY~ b) plot the maximum error ($\max_i F(x_i(k)) - F(x^*)$) vs the number of iterations confirming the known result that a smaller number of iterations is required to achieve a given precision with a denser topology. Finally, the combination of the two effects is in Fig.~YYY d), where we see that the expander with degree $20$ achieves the faster convergence in terms of time. This value is really close to the one predicted by our model ($d=18$!) and then confirms that the model can be effectively used to tune the topology of the dependency graph. In a multi-agent system (sensor network, robot team, etc.), every agent can be computing its own estimate with the purpose to use it, but in the case of ML distributed optimization, at the end of the optimization phase, the different local models can be aggregated to achieve a better model. In particular here we assume that the parameters of the aggregate model ($y(k)$) are simply the average of the local models: $y(k)=1/n\sum_{i=1}^n w_i(k)$. Figure YYY~d) shows how the error of the aggregate model ($F(y(k))-F(x^*)$) evolves as the number iterations increases.\footnote{
%	Note that while we show the error of the aggregate model at each iteration, the model would be actually computed only after the last iteration.
%} Qualitatively, we observe that the error decreases faster and that it is less dependant on the topology than the maximum error across the different local estimate. This result appears clearer in Fig.~ZZZ showing the slopes of the error vs iteration curves vs their theoretical values as computed by xxx. We observe that the smaller effect of the topology on the aggregate-model error has as consequence that sparser topology can be even more advantageous: \\
%\emph{Remark 1:~Aggregate models call for sparsity.} \\
%This is the first of a series of observations that will lead to the conclusion that the optimal topology can be even sparser than what our analysis in Sect. xxx suggests. 
%
%%We now modify our datasets increasing the value of $\zeta$ to $1$. Comparing Fig.~AAA and Fig.YYY~b) we see that the difference across the topologies is less evident in particular during the first iterations. This effect is similar to region of confusion...
%%\emph{Remark 2:~Clarity of direction calls for sparsity.} \\
%
%In the description above we have omitted to specify how the vector $\uv$ is selected. For each topology considered, $\uv$ is the eigenvector corresponding to $\lambda_2(P_n)$ with $||\uv||_\infty=1$ and smallest component equal to $-1$. Because $P_n$ is symmetric, $\uv$ is orthogonal to the unit vector, i.e. $\sum_i u_i=0$. This choice of $\uv$ corresponds to a worst case for the DSM algorithm as justified mathematically in \citeapp{a:worst_dataset}, and then to the case when the bound~\ref{e:error_bound2} is tighter. There is obviously no reason to assume that the dataset should be someway correlated to the dependency graph. We consider now a dataset generated by picking uniformly at random in $[-1,1]$ the feature values $\vx^{(l)}$ and selecting $y^{(l)}=- \sign(\vx^{(l)})$ with probability $0.95$ and $y^{(l)}=\sign(\vx^{(l)})$ with the complementary probability.
%Figure~BBB shows that 
%
%
%
%\emph{Remark 3:~Real datasets call for sparsity.}\\
%
%
%\emph{Remark 4:~Larger local datasets call for sparsity.}\\
%


